A Large-Scale Empirical Study of Quality Assurance Practices and Gaps in AI Agents

Large language model (LLM)-based agents are increasingly used across software engineering, web automation, research, and productivity applications. Their integration of planning, memory, tool use, code execution, and external interactions enables greater autonomy but also introduces new reliability, safety, and security risks. We present a large-scale empirical study of quality assurance (QA) practices in 157 open-source LLM-based agent projects with at least 100 GitHub stars. We analyze documentation, source code, configurations, and tests to characterize QA practices across execution surfaces, safeguards, testing artifacts, risk scenarios, and recurring gaps. We find that current QA primarily focuses on basic functionality and high-risk actions, while coverage remains fragmented. Safeguards are inconsistently applied across equivalent execution routes, tests rarely examine boundary, adversarial, or multi-step tool-use failures, and identified risks are seldom translated into end-to-end QA checks. These findings highlight the need to move beyond feature-level testing toward systematic end-to-end validation that ensures agent workflows remain within intended boundaries when interacting with untrusted inputs, tools, persistent state, and external APIs.

==> figures/figure1.tex <==
\begin{figure}[t!]  % Use [H] to enforce exact placement
    \centering
    \includegraphics[width=0.5\textwidth]{fig/overview-se-llm.png} % Adjust the path to the image
    \caption{Draft process}
    \label{fig:1}
\end{figure}

==> sec/approach.tex <==

%\section{Empirical Study Design}
%\label{sec:approach}

%Figure~\ref{fig:analysis-workflow} illustrates the overall workflow of our study, which consists of three stages: corpus selection, repository-level QA evidence review and annotation, and cross-repository synthesis.  In brief, our workflow first identifies open-source, runnable LLM-based agent applications, then reviews and annotates repository evidence according to the five QA dimensions, and finally aggregates the annotations to derive cross-repository statistics and recurring qualitative patterns.



\subsection{section{Research Questions}
\label{sec:rq}

We organize the study around five research questions.

\begin{description}[leftmargin=1.2cm, style=nextline]
  \item[RQ1.] What safety- and security-relevant execution surfaces and concern classes appear in existing LLM-based agent projects?
  \item[RQ2.] What testing artifacts and practices are used to evaluate agent safety and security?
  \item[RQ3.] What safeguards and prevention patterns are visible in repositories?
  \item[RQ4.] What safety and security risk scenarios emerge from observed model-to-tool execution surfaces?
  \item[RQ5.] What gaps exist between observed repository practices and the risks reported for LLM-based agents?
\end{description}

The questions separate concerns that are easy to conflate: exposed capabilities, tests, safeguards, risk scenarios, and remaining gaps. A project can document a risk without testing it; it can test a permission controller without applying that controller to every execution path; and it can expose a risky surface without containing a confirmed vulnerability. We therefore use the repository as the unit of analysis and do not reduce the study to vulnerability counting.


\subsection{Analysis Model}

We code each repository along five dimensions: architecture, execution surfaces, safeguards, testing artifacts, and risk scenarios. Together, they capture how an agent is organized, which privileged capabilities it exposes, how those capabilities are constrained, whether the boundaries are tested, and which evidence-backed risk chains are visible. The same dimensions guide manual review notes and aggregate tables, so the experiment section can focus on corpus construction and evidence collection rather than redefining the coding scheme. A potential risk observation is a repository-evidence note about a boundary question; it is not a confirmed vulnerability. Table~\ref{tab:analysis-dimensions} summarizes the rubric.

\begin{table}[htbp]
  \centering
  \scriptsize
  \caption{Analysis dimensions used across the study.}
  \label{tab:analysis-dimensions}
  \begin{tabularx}{\linewidth}{p{0.24\linewidth}X}
    \toprule
    Dimension & What we code and inspect \\
    \midrule
    Architecture & Agent control pattern, coordination, memory, and interface form from source structure, prompts, docs, and tool registries. \\
    Execution surface & Capability paths that can observe, mutate, execute, persist, or transmit data, including shell, files, browser, APIs, MCP/plugins, and secrets. \\
    Safeguard & Policy, approval, sandboxing, redaction, allow/deny lists, auth, and path checks in code, configuration, tests, or security docs. \\
    Testing artifact & Tests or evals related to safety/security boundaries, including permission, sandbox, adversarial, and benchmark paths. \\
    Risk scenario & Chain from entry point to model-influenced context or configuration to a sensitive sink, recorded as potential evidence rather than vulnerability proof. \\
    \bottomrule
  \end{tabularx}
\end{table}

% Removed visible terminology table to reduce space; the key distinctions are folded into the analysis-model paragraph and Table~\ref{tab:analysis-dimensions}.

\subsection{Architecture Coding}

Architecture labels are grounded in prior agent work on memory, planning, action, perception, and coordination \cite{wang2023surveyagents,xi2023rise}. We map repositories to implementation patterns such as ReAct loops \cite{yao2023react}, tool-router/MRKL-style agents \cite{karpas2022mrkl}, plan-execute or workflow-graph agents, reflection/tree-search agents \cite{shinn2023reflexion,yao2023tree,zhou2024lats}, and multi-agent systems \cite{wu2023autogen,li2023camel,hong2023metagpt,qian2023chatdev}.

Because projects often combine patterns, we retain secondary architecture evidence but report one primary pattern in corpus-level tables. Central multi-agent, tree-search, reflection, plan-execute, or workflow-graph designs take precedence; otherwise, observe-act loops are coded as ReAct-loop, and projects centered on function calling, tool registries, MCP, plugins, or external module routing are coded as tool-router/MRKL-inspired. Interface form is recorded separately because CLI, IDE, web, desktop, and messaging paths may enforce the same architecture differently.


==> sec/results.tex <==
\section{Results}
\label{sec:result}

\subsection{Descriptive Context: Corpus Architecture}

Table~\ref{tab:architecture-distribution} reports the primary architecture pattern assigned to each project. The two largest groups are tool-router/MRKL-inspired agents and ReAct-loop agents. In this corpus, the common implementation pattern is LLM-selected tools or iterative observe-act loops rather than full tree search, reflection memory, or explicit multi-agent protocols. Because this is a primary-label table, rare specialized patterns are grouped rather than shown as separate one-project rows; broader multi-agent and manager-worker behavior is reported in Table~\ref{tab:agent-components}.

\begin{table}[htbp]
  \centering
  \small
  \caption{Primary architecture patterns in the corpus.}
  \label{tab:architecture-distribution}
  \begin{tabularx}{0.82\linewidth}{Xrr}
    \toprule
    Architecture pattern & Repos. & Share \\
    \midrule
    Tool-router / MRKL-inspired & 78 & 49.7\% \\
    ReAct-loop & 44 & 28.0\% \\
    General tool agent & 20 & 12.7\% \\
    Plan-execute & 8 & 5.1\% \\
    Workflow-graph & 4 & 2.5\% \\
    Other specialized patterns & 3 & 1.9\% \\
    \bottomrule
  \end{tabularx}
\end{table}

The grouped ``Other specialized patterns'' row contains the three one-project primary labels: one role/SOP multi-agent system, one conversational multi-agent system, and one tree-search agent. We group them because Table~\ref{tab:architecture-distribution} is meant to summarize dominant primary designs, while Table~\ref{tab:agent-components} separately reports broader multi-agent and coordination evidence.

Table~\ref{tab:agent-components} reports additional architecture dimensions. Counts are normalized within each dimension and therefore each dimension sums to the corpus size; they are separate from the multi-label architecture evidence retained in the main CSV. Human-agent collaboration is common because many agents are interactive assistants with approval, review, or chat feedback. Reactive planning dominates, while explicit task decomposition appears in a smaller but prominent set of coding and workflow agents. Long-term memory and vector databases are less common than context-only or unspecified memory, suggesting that many projects prioritize tool execution over durable agent state.

\begin{table}[htbp]
  \centering
  \small
  \caption{Selected architecture dimensions.}
  \label{tab:agent-components}
  \begin{tabularx}{\linewidth}{p{0.18\linewidth}Xrr}
    \toprule
    Dimension & Label & Repos. & Share \\
    \midrule
    Topology & Human-agent collaboration & 80 & 51.0\% \\
    Topology & Hybrid multi-agent/human & 52 & 33.1\% \\
    Topology & Single-agent & 16 & 10.2\% \\
    Topology & Multi-agent & 9 & 5.7\% \\
    \addlinespace
    Planning & Reactive & 126 & 80.3\% \\
    Planning & Unspecified & 16 & 10.2\% \\
    Planning & Task decomposition & 13 & 8.3\% \\
    Planning & Workflow graph & 1 & 0.6\% \\
    Planning & Reflection & 1 & 0.6\% \\
    \addlinespace
    Memory & None or unspecified & 99 & 63.1\% \\
    Memory & Context-only & 43 & 27.4\% \\
    Memory & Long-term & 9 & 5.7\% \\
    Memory & Vector DB & 5 & 3.2\% \\
    Memory & Episodic reflection & 1 & 0.6\% \\
    \addlinespace
    Coordination & None or single-agent & 117 & 74.5\% \\
    Coordination & Manager-worker & 34 & 21.7\% \\
    Coordination & Workflow graph & 4 & 2.5\% \\
    Coordination & Conversation & 1 & 0.6\% \\
    Coordination & SOP pipeline & 1 & 0.6\% \\
    \bottomrule
  \end{tabularx}
\end{table}

These architecture results provide context for the five research questions below: most projects are tool-using, interactive agents, so safety and security depend on how model-mediated decisions connect to concrete execution surfaces, safeguards, tests, and end-to-end risk chains.

\subsection{RQ1: Execution Surfaces and Concern Classes}

RQ1 asks which safety- and security-relevant execution surfaces and concern classes appear in existing agent projects. In this corpus, the main concerns are broader than prompt quality alone. They come from capabilities that connect model-influenced behavior to commands, files, browsers, plugins, network APIs, dynamic code, secrets, and approval boundaries. Table~\ref{tab:surfaces} summarizes execution surfaces coded from structured review fields. A surface is marked present when repository evidence shows a code or configuration path for that capability: for example, shell tools or subprocess calls for shell/process execution, file APIs or workspace operations for filesystem access, Playwright/Selenium/browser state for browser automation, MCP server/client or plugin configuration for MCP/plugin mechanisms, provider keys or credential paths for secret handling, and authorization/approval/permission code for approval or auth boundaries. Surface presence does not by itself prove that the model can directly invoke that path.

\begin{table}[htbp]
  \centering
  \small
  \caption{Execution surfaces observed in 157 repositories.}
  \label{tab:surfaces}
  \begin{tabularx}{0.86\linewidth}{Xrr}
    \toprule
    Surface & Repos. & Share \\
    \midrule
    Network / API access & 156 & 99.4\% \\
    Secret handling & 155 & 98.7\% \\
    Filesystem access & 153 & 97.5\% \\
    Shell / command execution & 148 & 94.3\% \\
    Approval or auth boundary & 143 & 91.1\% \\
    MCP/plugin mechanism & 127 & 80.9\% \\
    Dynamic code or runtime loading & 123 & 78.3\% \\
    Browser automation & 119 & 75.8\% \\
    \bottomrule
  \end{tabularx}
\end{table}

These counts show that many repositories contain real execution capabilities, not only prompt or chat code. The common security question is therefore not only whether an LLM can produce unsafe text, but whether model-influenced text can reach a sensitive sink. Shell-enabled coding agents include command execution and package-install paths. Browser agents include pages, DOM state, screenshots, cookies, downloads, and remote debugging channels. MCP/plugin-enabled agents include additional tool registries and may inherit environment variables. Projects with custom OpenAI-compatible base URLs or provider routing include secret-forwarding decisions. Memory and session systems persist transcripts, tool outputs, and sometimes user secrets.

Concrete examples illustrate what these surfaces mean in repository evidence. In \texttt{google-gemini/gemini-cli}, the reviewed code exposes shell execution, workspace file operations, web fetch/search, browser-agent automation, MCP extensions, and an A2A server package; the corresponding review notes identify YOLO/allow policies, trusted MCP servers, and non-interactive consent as places where approval behavior can change. In \texttt{OpenHands/OpenHands}, a software-engineering agent provisions a workspace sandbox and routes conversations to an agent server with file, shell, browser, MCP, and plugin capabilities; the relevant quality question is how sandbox isolation, local API exposure, setup hooks, and user-provided secrets interact. In \texttt{NousResearch/hermes-agent}, a general-purpose assistant combines terminal backends, file tools, browser automation, plugins, MCP, memory, and messaging gateways, so the enforcement points span both local runtime and channel adapters.

The structured reviews contain 814 potential risk observations across 156 repositories. These observations are evidence-backed notes rather than confirmed vulnerabilities, and the tag counts should be read as signals about what reviewers had to inspect, not as vulnerability prevalence. Table~\ref{tab:risk-tags} reports the most frequent normalized tags; tags were case-normalized and obvious aliases such as MCP and MCP/plugin were merged.

\begin{table}[htbp]
  \centering
  \small
  \caption{Most frequent tags in structured risk observations.}
  \label{tab:risk-tags}
  \begin{tabularx}{0.72\linewidth}{Xrr}
    \toprule
    Tag & Observations & Share \\
    \midrule
    Secrets & 405 & 49.8\% \\
    Approval / policy & 388 & 47.7\% \\
    Execution & 330 & 40.5\% \\
    Filesystem & 254 & 31.2\% \\
    MCP/plugin & 199 & 24.4\% \\
    Supply chain & 176 & 21.6\% \\
    Application API & 144 & 17.7\% \\
    Dynamic code & 133 & 16.3\% \\
    Network & 120 & 14.7\% \\
    Browser & 101 & 12.4\% \\
    \bottomrule
  \end{tabularx}
\end{table}

\mybox{\textbf{Answer to RQ1.} Existing LLM-agent projects commonly expose high-authority execution surfaces: network/API access, secrets, filesystem operations, shell/process execution, approval/auth boundaries, MCP/plugin mechanisms, dynamic code loading, and browser automation. The dominant concern classes are model-to-tool execution, filesystem and shell authority, plugin/MCP trust, browser/session exposure, provider-secret routing, approval bypass, and persistence of sensitive state.}

\subsection{RQ2: Testing Artifacts and Practices}

RQ2 examines visible testing files and practices for agent safety and security. We separate ordinary software tests from files that appear to exercise safety, security, policy, sandboxing, authentication, secret handling, or adversarial behavior. Table~\ref{tab:testing-artifacts} reports a reproducible path-based count generated from repository snapshots. These counts are heuristic: they measure the presence of likely files, not the quality or completeness of the tests.

\begin{table}[htbp]
  \centering
  \small
  \caption{Path-based testing and review files in repository snapshots.}
  \label{tab:testing-artifacts}
  \begin{tabularx}{\linewidth}{XrrX}
    \toprule
    Artifact class & Repos. & Share & Predicate summary \\
    \midrule
    Any tests or specs & 137 & 87.3\% & Test/spec directory or conventional test/spec filename. \\
    Security/safety tests & 95 & 60.5\% & Test/spec path plus safety, security, permission, sandbox, auth, secret, guard, approval, policy, or prompt-injection term. \\
    Eval/red-team-like files & 73 & 46.5\% & Eval, benchmark, red-team, jailbreak, adversarial, or prompt-injection path. \\
    Security/safety docs or code & 126 & 80.3\% & Security, safety, sandbox, permission, threat, auth, or secret basename. \\
    \bottomrule
  \end{tabularx}
\end{table}

The clearest safety and security testing patterns appear in manually inspected coding and browser agents with larger test suites. Examples in the corpus include tests for command approval, sandbox recovery, browser policy, domain filtering, structured sandbox outputs, authentication, token handling, and permission isolation. Some projects also maintain evaluation suites for tool use, automated actions, browser tasks, or agent behavior under constrained environments. These tests are valuable because they encode concrete boundaries rather than relying on documentation alone.

For example, \texttt{google-gemini/gemini-cli} contains explicit safety boundaries around shell execution, workspace containment, browser consent, and MCP trust, so its tests and review evidence can be mapped to concrete agent behaviors such as command approval and browser access. \texttt{OpenHands/OpenHands} provides another pattern: tests and review evidence are tied to sandboxed software-engineering workflows, where repository setup, workspace persistence, browser tools, and local API assumptions all affect the same agent run. These are qualitatively different from a simple unit test that only checks whether a function returns a value.

However, many reviewed tests are functional rather than adversarial. They check that a tool works, an integration returns a result, or a UI state changes, but not whether a malicious prompt, web page, repository file, plugin, or subagent can drive the tool across a security boundary. This distinction matters for agents because the adversary may be indirect. An untrusted webpage, issue comment, README, dependency script, MCP tool description, or retrieved document can become part of the model context and influence later actions.

\mybox{\textbf{Answer to RQ2.} Most repositories contain conventional tests, and many contain safety/security-related files, but the visible practice is uneven. The strongest evidence is component-level testing of permissions, sandboxes, authentication, command approval, browser policy, token handling, and tool behavior; end-to-end adversarial tests are less visible.}

\subsection{RQ3: Safeguards and Prevention Patterns}

RQ3 asks what safeguards and prevention patterns are visible in repositories. We use ``safeguard'' broadly: code, configuration, policy, or runtime checks that reduce unsafe behavior before or during tool execution. Table~\ref{tab:mechanism-artifacts} reports path-based evidence for files related to those safeguards. These counts should be read as repository evidence counts, not proof that each safeguard is complete, active by default, or consistently enforced.

\begin{table}[htbp]
  \centering
  \small
  \caption{Safeguard-related files in repository snapshots.}
  \label{tab:mechanism-artifacts}
  \begin{tabularx}{\linewidth}{XrrX}
    \toprule
    Artifact class & Repos. & Share & Predicate summary \\
    \midrule
    MCP/plugin files & 108 & 68.8\% & MCP/plugin path. \\
    Sandbox / isolation files & 107 & 68.2\% & Sandbox, container, Docker, isolation, jail, or chroot path. \\
    Permission / policy files & 104 & 66.2\% & Permission, approval, policy, allowlist, denylist, or guard path. \\
    Secret / redaction files & 99 & 63.1\% & Secret, credential, token, redaction, masking, or sanitization path. \\
    Browser / domain files & 92 & 58.6\% & Browser, domain, cookie, origin, CORS, URL allow, or URL block path. \\
    \bottomrule
  \end{tabularx}
\end{table}

Across the reviewed repositories, visible safeguard evidence includes approval policies, sandboxes, allow/deny lists, path checks, secret redaction, provider URL checks, plugin provenance checks, and local API authentication or CSRF controls. These are evidence categories, not validated enforcement guarantees. In manually inspected examples, coding agents include command or file approval logic, browser agents include browser isolation, domain policy, or session-handling code, and SWE automation agents include container, subprocess, or remote workspace isolation. Several larger projects also include secret redaction in settings APIs, logs, telemetry, and model/tool messages.

The same safeguard category can look very different across repositories. \texttt{Kilo-Org/kilocode} has permission prompts and rule evaluation for shell and file tools, but review evidence also records automation modes such as \texttt{--auto}, saved wildcard rules, and \texttt{/allow-everything}. \texttt{lobehub/lobehub} has a central intervention engine with manual, allow-list, auto-run, and headless modes, while desktop filesystem and shell handlers rely partly on upstream approval decisions. \texttt{RooCodeInc/Roo-Code} centralizes approvals for tool use, but its review notes point to alternate paths such as MCP always-allow settings, custom tools, CLI/eval auto-approval, wildcard command allowlists, and outside-workspace toggles. These are not identical bugs; they are examples of why safeguard coverage must be checked across execution paths.

The main qualitative pattern is inconsistency across execution paths. A permission model may be carefully implemented for the interactive UI while a non-interactive CLI flag, local API endpoint, background worker, subagent, or test/eval harness uses a different path. MCP/plugin systems add another layer: a project can have strong built-in tool approvals while allowing user-configured stdio MCP servers or plugin sources to introduce new callable tools with their own process, network, and secret behavior. Similarly, a sandbox can protect the host while still exposing repository secrets, browser cookies, mounted workspaces, or provider keys inside the agent environment.

\mybox{\textbf{Answer to RQ3.} The visible prevention patterns are approval gates, permission policies, sandboxing and container isolation, allow/deny lists, path checks, secret redaction, provider or URL checks, authentication controls, and plugin/MCP constraints. The recurring weakness is inconsistent coverage across UI, CLI, API, plugin, subagent, setup, and evaluation paths.}

\subsection{RQ4: Safety and Security Risk Scenarios}

RQ4 organizes concrete risk scenarios that emerge from the observed execution surfaces. We define a scenario as a chain from an entry point, through model-influenced context or configuration, to a sensitive sink. We do not treat a scenario as a confirmed vulnerability unless repository evidence shows reachability and an insufficient boundary. Table~\ref{tab:risk-scenarios} summarizes the qualitative scenario taxonomy and the coded fields used for interpretation; the scenarios below are risk patterns that help compare projects.

\begin{table}[htbp]
  \centering
  \small
  \caption{Qualitative risk-scenario taxonomy and coded evidence fields used for interpretation.}
  \label{tab:risk-scenarios}
  \begin{tabularx}{\linewidth}{p{0.34\linewidth}X}
    \toprule
    Scenario & Evidence source used in this study \\
    \midrule
    Prompt/content to file access & Filesystem surface; prompt-injection and filesystem tags \\
    Model output to shell execution & Shell surface; execution and approval tags \\
    Browser task to session exposure & Browser surface; browser, network, and secrets tags \\
    MCP/plugin to process execution & MCP/plugin surface; MCP/plugin, execution, supply-chain tags \\
    Provider routing to secret forwarding & Secret surface; secrets and network tags \\
    Memory/transcript persistence & Qualitative review evidence; secrets, filesystem, and persistence-related tags \\
    \bottomrule
  \end{tabularx}
\end{table}

\textbf{Prompt or content injection to filesystem access.} Coding agents and research agents often read repository files, issue content, documentation, webpages, or retrieved documents into context. If those inputs instruct the model to read credential files, hidden configuration, transcripts, or browser state, the critical question is whether the file tool enforces workspace containment and whether secret-like files are excluded from model-visible output.

For example, \texttt{RooCodeInc/Roo-Code} exposes file read/write/edit/search tools with optional outside-workspace access; the review evidence records protected configuration checks but also support for absolute paths and outside-workspace toggles when approved or auto-approved. \texttt{NousResearch/hermes-agent} similarly exposes broad file tools with redaction and denylist logic, but no default project-root containment for reads and writes. These examples fall under the prompt/content-to-filesystem scenario because untrusted context can influence what the agent asks the file tool to read.

\textbf{Model output to shell execution.} Shell tools are present in 148 repositories. The risk is not simply that shell execution exists; it is whether shell execution is gated consistently. Review observations include approval-related and execution-related tags, including paths where full-auto, eval, subagent, setup-hook, package-manager, or configured-command behavior may differ from a normal interactive approval loop.

For example, \texttt{OpenHands/OpenHands} review evidence records repository-controlled setup scripts that execute during conversation startup, before the agent's normal task loop. \texttt{zgsm-ai/costrict} provides a contrasting coding-agent example where model output can reach shell execution and several CLI or review modes auto-handle approvals. Both examples are shell-execution scenarios, but one centers on startup/setup behavior while the other centers on approval defaults and alternate run modes.

\textbf{Browser task to session exposure.} Browser/computer-use agents can observe DOM content, screenshots, URLs, downloads, cookies, and local storage depending on implementation. Malicious pages can act as indirect prompt-injection sources \cite{greshake2023indirect,liu2023houyi}. The relevant boundary is whether browser state is isolated per task, whether sensitive domains are excluded, whether downloads and uploads are scoped, and whether page content can instruct the agent to use unrelated tools.

For example, \texttt{google-gemini/gemini-cli} includes optional browser automation where existing or persistent browser modes can expose signed-in state, and the review notes identify non-interactive consent behavior as a boundary to inspect. \texttt{browser-use/browser-use} exposes an LLM-driven browser agent that observes DOM, screenshot, and file state and executes browser actions through its controller; the relevant boundary is how task content, browser state, downloads, and custom tools are scoped.

\textbf{MCP/plugin configuration to local process execution.} MCP/plugin mechanisms appear in 127 repositories. Stdio MCP servers are especially important because they are both tool surfaces and process-execution surfaces. If users, repositories, or remote plugin metadata can define commands, arguments, or environment variables, then plugin provenance and environment minimization become security-critical.

For example, \texttt{Kilo-Org/kilocode} and \texttt{RooCodeInc/Roo-Code} both allow MCP configuration to register local stdio commands. The review evidence for both projects records environment inheritance and approval/always-allow settings as the relevant boundaries. \texttt{anomalyco/opencode} shows a related local-assistant pattern: configured MCP servers and plugins can add model-callable tools while inheriting process and workspace context.

\textbf{Custom provider routing to secret forwarding.} Projects with OpenAI-compatible base URLs, multiple providers, proxy endpoints, or custom model gateways create a secret-routing boundary. Provider keys can be exposed to non-provider endpoints if URL validation, private-network blocking, or per-provider key scoping is weak.

For example, \texttt{google-gemini/gemini-cli}, \texttt{OpenHands/OpenHands}, and \texttt{NousResearch/hermes-agent} all support multiple model providers or OpenAI-compatible endpoints. The review evidence does not treat provider flexibility as a bug by itself; it records where provider keys, custom base URLs, subprocess environments, MCP environment variables, or ACP/plugin contexts can receive secrets.

\textbf{Memory, transcript, and telemetry persistence.} Agent memory can preserve useful context, but it can also persist sensitive tool outputs, user secrets, repository data, or browser observations. We treat this as a qualitative risk scenario rather than a separately counted execution surface. Redaction after persistence is weaker than redaction before storage and before model-visible reuse. The risk increases when memories are shared across projects, subagents, or plugin contexts.

For example, \texttt{anomalyco/opencode} and \texttt{OpenHands/OpenHands} both persist sessions and workspace-related state while exposing file, shell, and plugin tools. In these projects, the review question is not merely whether memory exists, but whether transcripts, tool outputs, settings, and secret references are redacted before storage and before later model-visible reuse.

\mybox{\textbf{Answer to RQ4.} The main risk scenarios are prompt/content to file access, model output to shell execution, browser task to session exposure, MCP/plugin configuration to process execution, provider routing to secret forwarding, and memory/transcript persistence. These are risk chains inferred from repository evidence, not confirmed vulnerabilities.}

\subsection{RQ5: Gaps Between Practice and Risk}

RQ5 synthesizes gaps between practices observed in this corpus and the risks exposed by LLM-based agents. The gaps are not uniform across projects. Some repositories have mature policies and tests; others are early prototypes. The recurring issue is that capability evidence is often broader than enforcement evidence.

\textbf{Gap 1: tool authority can be broader than policy authority.} Agents in the corpus commonly include shell, filesystem, browser, network, and plugin surfaces, but the policy layer can be narrower than the tool layer. A project may have a command approval UI while leaving MCP tools, setup hooks, background workers, or custom agent commands governed by separate logic. This creates policy fragmentation.

In \texttt{Kilo-Org/kilocode}, for instance, the same agent can expose shell, filesystem, browser-via-MCP, plugin, and local server surfaces, while automation flags and broad allow rules change when human review occurs. In \texttt{anomalyco/opencode}, shell/file tools route through permissions, but the reviewed evidence also records HTTP session and permission-control endpoints, MCP tools, plugins, and PTY surfaces. These examples show policy fragmentation: the relevant question is whether every path to the same authority is governed by the same policy.

\textbf{Gap 2: interface paths are treated as deployment details, but they change risk.} Architecture and interface are different, but interfaces still matter for enforcement. A ReAct coding agent exposed through a local web app, CLI, IDE extension, API server, and subagent worker can have several different auth, approval, and logging paths. Safety claims should therefore be checked across all interfaces, not only the primary demo path.

\texttt{OpenHands/OpenHands} illustrates this gap because local OSS deployments, sandboxed agent-server execution, browser tools, plugin/MCP configuration, and optional API/session settings create different trust assumptions. \texttt{NousResearch/hermes-agent} has CLI, TUI, dashboard, gateway, OpenAI-compatible API, browser, terminal, plugin, and MCP paths; review notes identify dashboard plugin routes and non-interactive/container execution as places where approval and auth assumptions differ from the main interactive path.

\textbf{Gap 3: plugin ecosystems blur the trusted computing base.} MCP servers, skills, hooks, extensions, and remote plugin metadata let agents grow capabilities after installation. This is useful, but it means the trusted computing base includes plugin discovery, provenance, command spawning, environment inheritance, and tool descriptions. In the reviewed projects, plugin onboarding is often easier to identify than explicit constraint documentation.

\texttt{lobehub/lobehub}, \texttt{RooCodeInc/Roo-Code}, and \texttt{Kilo-Org/kilocode} all show this pattern in different forms: desktop MCP configs can start stdio commands, marketplace or project settings can install or enable tools, and model-visible tool descriptions become part of the agent's action space. The gap is not that plugin ecosystems are inherently unsafe; it is that their provenance, environment, and approval boundaries need to be documented and tested as part of the agent, not treated as external add-ons.

\textbf{Gap 4: browser and retrieval agents inherit indirect prompt-injection risk.} Prior work shows that external content can manipulate LLM-integrated applications \cite{greshake2023indirect,liu2024formalizing}. Browser agents make this risk operational because page content can be followed by tool use. Domain filters and browser sandboxes help, but session, cookie, upload, download, and cross-domain policies are not consistently explicit in repository evidence.

\texttt{google-gemini/gemini-cli} and \texttt{browser-use/browser-use} illustrate two variants. In the former, browser automation can be connected to existing or persistent browser state depending on configuration; in the latter, browser task content flows through an LLM-driven browser controller. Both cases require policies about page content, domains, downloads, and whether browser observations can trigger unrelated tools.

\textbf{Gap 5: tests lag behind adversarial chains.} Safety-related tests exist in many repositories, but they often test components independently. Agent failures frequently require chains: a malicious README affects planning, planning calls a shell tool, the shell tool sees secrets in environment, and logs persist the result. End-to-end adversarial tests for these chains are less common than unit tests for individual tools.

For example, a repository may test command approval and separately test secret redaction, but not the chain in which untrusted repository content asks the model to call a shell tool that inherits provider keys and writes output into a persistent transcript. The reviewed evidence for \texttt{google-gemini/gemini-cli}, \texttt{Kilo-Org/kilocode}, and \texttt{OpenHands/OpenHands} shows enough individual boundaries to inspect such chains, but the corpus-level pattern is that end-to-end adversarial coverage is harder to see than component-level tests.

The practical implication is that agent safety work should check complete execution paths, not just individual features. A project should be able to answer where each agent-exposed tool is registered, what authority it receives, what untrusted context can influence it, which approval or policy checks apply, where outputs are stored, and whether the same answer holds for UI, CLI, API, plugin, subagent, and eval paths.

\mybox{\textbf{Answer to RQ5.} The central gap is that agent capabilities are broader and more compositional than the visible quality-assurance evidence. Policies often cover the main interactive path but not every interface, and tests often validate individual components rather than adversarial chains across context, tools, secrets, and persistence.}


